Community Smells -- The Sources of Social Debt: A Systematic Literature Review

Context: Social debt describes the accumulation of unforeseen project costs (or potential costs) from sub-optimal software development processes. Community smells are sociotechnical anti-patterns and one source of social debt that impact software teams, development processes, outcomes, and organizations. Objective: To provide an overview of community smells based on published literature, and describe future research. Method: We conducted a systematic literature review (SLR) to identify properties, understand origins and evolution, and describe the emergence of community smells. This SLR explains the impact of community smells on teamwork and team performance. Results: We include 25 studies. Social debt describes the impacts of poor socio-technical decisions on work environments, people, software products, and society. For each of the 30 identified community smells, we provide a description, management approaches, organizational strategies, and mitigation effectiveness. We identify five groups of management approaches: organizational strategies, frameworks, models, tools, and guidelines. We describe 11 properties of community smells. We develop the Community Smell Stages Framework to concisely describe the origin and evolution of community smells. We describe the causes and effects for each community smell. We identify and describe 8 types of causes and 11 types of effects for community smells. Finally, we provide 8 Sankey diagrams that offer insights into threats the community smells pose to teamwork factors and team performance. Conclusion: Community smells explain the influence work conditions have on software developers. The literature is scarce and focuses on a small number of community smells. Thus, community smells still need more research. This review organizes the state of the art about community smells and provides motivation for future research along with educational material.

==> tables/table_CSsTeamworkConsiderations.tex <==
  \multirow{3}{*}{Community-smell name} & \multicolumn{8}{c|}{Critical Considerations of Teamwork}\\
\cline{2-9}
  & \multicolumn{5}{c|}{Core processes and emergent states} & \multicolumn{3}{c|}{Influencing conditions}\\
\cline{2-9}
  & Cognition & Communication & Conflict & Cooperation & Coordination & Composition & Context & Culture\\
  \hline
 \endfirsthead
\hline
 \multicolumn{9}{c}
 {{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline
  \multirow{3}{*}{Community-smell name} & \multicolumn{8}{c|}{Critical Considerations of Teamwork}\\
\cline{2-9}
  & \multicolumn{5}{c|}{Core processes and emergent states} & \multicolumn{3}{c|}{Influencing conditions}\\
\cline{2-9}
  & Cognition & Communication & Conflict & Cooperation & Coordination & Composition & Context & Culture\\ 
 \endhead
\hline
 \multicolumn{9}{r}{{Continued on next page}} \\ \hline
\endfoot
\hline
\endlastfoot

Architecture by osmosis & & \cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& & & \cellcolor{black!10}\checkmark& \\
\hline

Architecture hood & & & & \cellcolor{black!10}\checkmark& & & & \\
\hline

Black cloud & & \cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& & & & \\
\hline

Class cognition & & & & & \cellcolor{black!10}\checkmark& & & \\
\hline

Code red & & & & & \cellcolor{black!10}\checkmark& & & \\
\hline

Cognitive distance & \cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& \\
\hline

Cookbook development & \cellcolor{black!10}\checkmark& & & & & & & \\
\hline

DevOps clash & & \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& & & \cellcolor{black!10}\checkmark\\
\hline

Disengagement & \cellcolor{black!10}\checkmark& & & & & & & \\
\hline

Dispersion & & & & & \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& & \\
\hline

Dissensus & & & \cellcolor{black!10}\checkmark& & & & & \\
\hline

Hyper community & & & \cellcolor{black!10}\checkmark& & & & & \\
\hline

Informality excess & & \cellcolor{black!10}\checkmark& & & & & \cellcolor{black!10}\checkmark& \\
\hline

Institutional isomorphism & & \cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& \\
\hline

Invisible architecting & \cellcolor{black!10}\checkmark& & & & & & \cellcolor{black!10}\checkmark& \\
\hline

Leftover techie & & \cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& & & & \\
\hline

Lone wolf & & & & \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& & & \\
\hline

Lonesome architecting &\cellcolor{black!10}\checkmark& & & & & & \cellcolor{black!10}\checkmark& \\
\hline

Newbie free-riding & & & \cellcolor{black!10}\checkmark& & & & \cellcolor{black!10}\checkmark& \\
\hline

Obfuscated architecting & &\cellcolor{black!10}\checkmark& & & & & \cellcolor{black!10}\checkmark& \\
\hline

Organizational silo & &\cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& \\
\hline

Organizational skirmish & & & & & \cellcolor{black!10}\checkmark& & & \\
\hline

Power distance & & & & & & & & \\
\hline

Priggish members & & & \cellcolor{black!10}\checkmark& & & & & \\
\hline

Prima donnas & &\cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& & & \\
\hline

Radio silence or Bottleneck & &\cellcolor{black!10}\checkmark& & & & & & \\
\hline

Sharing villainy & &\cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& & & & \\
\hline

Solution defiance & & & \cellcolor{black!10}\checkmark& \cellcolor{black!10}\checkmark& & & & \\
\hline

Time warp & & & & & \cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& \\
\hline

Unlearning &\cellcolor{black!10}\checkmark&\cellcolor{black!10}\checkmark& & \cellcolor{black!10}\checkmark& & & & 

==> tables/table_researchQuestions.tex <==
\centering
\begin{tabular}{ p{0.5cm} p{11.5cm} }
 \hline
 \textbf{RQ} & \textbf{Question's text} \\  
 \hline
 1 & What are the properties of the community smells?\\
 \hline
 2 & How do the community smells affect software development teams?\\
 \hline
 3 & Do the community smells emerge and generate effects that lead to Social Debt similarly?\\
 \hline
 4 & What are the most frequent types of causes behind the emergence of community smells and the types of effects?\\ 
 \hline
 5 & How do the community smells may affect teamwork in software development teams?\\
 \hline 
\end{tabular}

==> tables/table_selectionRelevantStudies.tex <==
\centering
\begin{tabular}{ l r r }
 \hline
 \rowcolor{Gray}
 \textbf{Step} & \textbf{Exclusions} & \textbf{Inclusions}\\ 
 \hline 
 Search and retrieval from digital libraries & - & 72\\
 Selection based on study titles & 42 & 30\\
 Exclusion based on abstract, keywords and conclusions & 3 & 27\\
 Exclusion based on extended abstracts & 2 & 25\\
 Exclusion of magazine articles & 2 & 23\\ 
 Exclusion based on full-text & 8 & 15\\
 %Studies reported in the SMS & 9 & 9\\
 \textbf{Total} & & \textbf{15}\\
 \hline
\end{tabular}
